Efficient Trajectory Forecasting and Generation with Conditional Flow Matching

Trajectory prediction and generation are crucial for autonomous robots in dynamic environments. While prior research has typically focused on either prediction or generation, our approach unifies these tasks to provide a versatile framework and achieve state-of-the-art performance. While diffusion models excel in trajectory generation, their iterative sampling process is computationally intensive, hindering robotic systems' dynamic capabilities. We introduce Trajectory Conditional Flow Matching (T-CFM), a novel approach using flow matching techniques to learn a solver time-varying vector field for efficient, fast trajectory generation. T-CFM demonstrates effectiveness in adversarial tracking, real-world aircraft trajectory forecasting, and long-horizon planning, outperforming state-of-the-art baselines with 35% higher predictive accuracy and 142% improved planning performance. Crucially, T-CFM achieves up to 100$\times$ speed-up compared to diffusion models without sacrificing accuracy, enabling real-time decision making in robotics. Codebase: https://github.com/CORE-Robotics-Lab/TCFM

==> 4_summary.tex <==
\subsection{Summary}

\feedback{Our experiments showcase \smodel's capacity to produce samples that surpass the performance of leading forecasting and tracking models in sparse adversarial settings as well as with real-world flight trajectory data. Furthermore, we illustrate that \smodel can generate long-horizon plans with sampling times that are an order of magnitude lower than previous methods. T-CFM paves the way for learned dynamic planning in real-world robots.}

% \feedback{Our experiments demonstrate the ability for \smodel to generate samples that outperform the best forecasting and tracking algorithms in both sparse adversarial settings and for real-world trajectory data. We additionally show that \smodel is capable of generating long-horizon plans with an order of magnitude lower sampling time than prior methods. T-CFM opens the way for learned dynamic replanning in real-world robots.}

% \feedback{Our experiments demonstrate that T-CFM consistently outperforms state-of-the-art baselines across diverse tasks, including adversarial tracking, aircraft trajectory forecasting, and long-horizon planning. In the adversarial tracking domain, T-CFM achieves up to a 17\% increase in predictive accuracy compared to prior methods (Table I). For aircraft trajectory forecasting, T-CFM surpasses FlightBERT with an average improvement of 35.4\% across all metrics (Table II). In long-horizon planning, T-CFM significantly outperforms Diffuser, achieving a 142\% increase in score when using just a single sampling step (Table III). Notably, T-CFM maintains its performance even when reducing the number of sampling steps (Figure 4b, Figure 6), enabling substantial speed-ups compared to diffusion-based models without compromising accuracy. Furthermore, T-CFM demonstrates the ability to generate high-quality trajectory samples with as few as one sampling step (Figure 4b, Table III), showcasing its efficiency and versatility.}

==> prisoner_table.tex <==

% With COLUMN DIVIDER
\setlength{\tabcolsep}{3pt}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{5}}

\begin{table*} \centering
\vspace{0.2cm}
\begin{tabular}{@{}lrrr|rrr|rrr|rrr@{}}
\toprule
Prisoner-Low \\
\toprule
& \multicolumn{3}{c}{} & \multicolumn{3}{c}{Log-Likelihood}& \multicolumn{3}{c}{$ADE$}& \multicolumn{3}{c}{CT$_\delta$} \\
\cmidrule{5-7} \cmidrule{8-10} \cmidrule{11-13}
& GNN  & $\omega$MM & MI & $0$ min & $30$ min & $60$ min & $0$ min & $30$ min & $60$ min & $0$ min & $30$ min & $60$ min \\ \midrule
 % & \multicolumn{1}{c}{GNN} & $\omega$MM & \multicolumn{1}{c}{MI} &       &       &       &       &       &       &       &       &       \\

% \textbf{Baselines}\\
LSTM                & -          & -          & -          & 4.901          & 4.135          & 2.843          & 0.069          & 0.090          & 0.136          & 0.910          & 0.844          & 0.728          \\
VRNN Seq            & -          & -          & -          & 4.421          & 4.217          & 3.850          & 0.106          & 0.093          & 0.119          & 0.738          & 0.677          & 0.610          \\
VAE Opponent        & -          & -          & -          & 5.121          & 3.973          & 3.685          & 0.085          & 0.095          & 0.119          & 0.723          & 0.600          & 0.561          \\
% \textbf{Our Approaches}\\
Ours (w/o GNN \& MI) & -          & \checkmark & -          & 5.784          & 5.504          & 4.460          & \textbf{0.060} & 0.083          & \textbf{0.109} & 0.958          & 0.916          & 0.891          \\
Ours (w/o GNN)      & -          & \checkmark & \checkmark & \textbf{6.381} & \textbf{5.606} & \textbf{4.702} & \textbf{0.060} & \textbf{0.080} & 0.110          & \textbf{0.960} & \textbf{0.925} & \textbf{0.902} \\
\midrule
\textbf{Includes Agent Position} \\
Ours (w/o MI)       & \checkmark & \checkmark & -          & 4.609          & \uline{5.071}    & 4.117          & 0.062          & 0.082          & 0.112          & \uline{0.960}    & \uline{0.926}    & \uline{0.876}    \\
Ours                & \checkmark & \checkmark & \checkmark & \uline{5.230}    & 4.845          & \uline{4.789}    & \uline{0.061}    & \uline{0.081}    & \uline{0.107}    & 0.957          & 0.931          & 0.857         \\

\bottomrule
\bottomrule

\toprule
Prisoner-Medium \\
\toprule
& \multicolumn{3}{c}{} & \multicolumn{3}{c}{Log-Likelihood}& \multicolumn{3}{c}{$ADE$}& \multicolumn{3}{c}{CT$_\delta$} \\
\cmidrule{5-7} \cmidrule{8-10} \cmidrule{11-13}
& GNN  & $\omega$MM & MI & $0$ min & $30$ min & $60$ min & $0$ min & $30$ min & $60$ min & $0$ min & $30$ min & $60$ min \\ \midrule

% \textbf{Baselines}\\
LSTM                & -          & -          & -          & 5.858                     & 4.091          & 2.836          & 0.066                     & 0.088          & 0.125          & 0.918                     & 0.830          & 0.618          \\
VRNN Seq            & -          & -          & -          & \multicolumn{1}{r}{3.732} & 4.214          & 3.599          & \multicolumn{1}{r}{0.172} & 0.086          & \textbf{0.110} & \multicolumn{1}{r}{0.495} & 0.666          & 0.553          \\
VAE Opponent        & -          & -          & -          & \multicolumn{1}{r}{5.432} & 4.372          & 3.281          & \multicolumn{1}{r}{0.063} & 0.080          & 0.117          & \multicolumn{1}{r}{0.734} & 0.665          & 0.445          \\
% \textbf{Our Approaches}\\
Ours (w/o GNN \& MI) & -          & \checkmark & -          & 7.214          & 5.065          & 4.256          & \textbf{0.047} & 0.078          & \textbf{0.110} & \textbf{0.973} & 0.939          & 0.883          \\
Ours (w/o GNN)       & -          & \checkmark & \checkmark & \textbf{7.981} & \textbf{5.288} & \textbf{4.385} & 0.049          & \textbf{0.077} & \textbf{0.110} & 0.965          & \textbf{0.952} & \textbf{0.901} \\
\midrule
\textbf{Includes Agent Position}\\
Ours (w/o MI)        & \checkmark & \checkmark & -          & 7.026          & 4.970          & \uline{4.109}    & \uline{0.048}    & 0.078          & \uline{0.113}    & 0.969          & 0.922          & 0.882          \\
Ours                 & \checkmark & \checkmark & \checkmark & \uline{8.406}    & \uline{5.270}    & 4.059          & 0.049          & \uline{0.073}    & \uline{0.113}    & \uline{0.972}    & \uline{0.943}    & \uline{0.898}  \\

\bottomrule
\bottomrule

\toprule
Prisoner-High \\
\toprule
& \multicolumn{3}{c}{} & \multicolumn{3}{c}{Log-Likelihood}& \multicolumn{3}{c}{$ADE$}& \multicolumn{3}{c}{CT$_\delta$} \\
\cmidrule{5-7} \cmidrule{8-10} \cmidrule{11-13}
& GNN  & $\omega$MM & MI & $0$ min & $30$ min & $60$ min & $0$ min & $30$ min & $60$ min & $0$ min & $30$ min & $60$ min \\ \midrule

% \textbf{Baselines}\\
LSTM                & -          & -          & -          & 6.955                     & 4.110          & 2.555                     & 0.042                     & 0.059          & 0.111                     & 0.946                     & 0.823          & 0.528                     \\
VRNN Seq            & -          & -          & -          & \multicolumn{1}{r}{5.037} & 4.345          & 2.967                     & \multicolumn{1}{r}{0.105} & 0.059          & 0.100            & \multicolumn{1}{r}{0.714} & 0.731          & 0.538                     \\
VAE Opponent        & -          & -          & -          & 2.991 & 4.172          & 2.754 & 0.200 & \textbf{0.054}          & 0.123 & 0.528 & 0.657          & 0.382 \\

% \textbf{Our Approaches}\\
Ours (w/o GNN \& MI) & -          & \checkmark & -          & 8.515  & 4.422          & \textbf{3.297} & 0.016 & 0.057 & 0.095 & \textbf{0.965} & 0.923          & \textbf{0.803} \\
Ours (w/o GNN)      & -          & \checkmark & \checkmark & \textbf{10.862} & \textbf{4.535} & 3.221          & \textbf{0.015} & 0.056          & \textbf{0.092} & 0.953 & \textbf{0.932} & 0.801          \\
\midrule
\textbf{Includes Agent Position}\\

Ours (w/o MI)       & \checkmark & \checkmark & -          & 8.346           & \uline{4.518}    & 3.147          & 0.018          & 0.049          & 0.098          & 0.965          & 0.892          & 0.753          \\
Ours                & \checkmark & \checkmark & \checkmark & \uline{11.094}    & 4.389          & 3.202          & \uline{0.015}    & \uline{0.046}    & \uline{0.092}    & \uline{0.970}    & \uline{0.910}          & \uline{0.795}           \\

\bottomrule
\end{tabular}


\caption{Prison Escape Environment Results for different prediction horizons. Underlined and bolded indicate the best models with and without agent positions, respectively}

\label{tab:prisoner}
\end{table*}
